The Company a Question Keeps: Auditing Open Jev-Style Models for Retrieval

Jev's documented interface evaluates typed questions independently against shared evidence. We audit request independence in seven open Jev-style checkpoints on 276 constructed three-passage states from 92 TREC retrieval queries. Paired interventions separately change requested questions, displayed evidence, and candidate eligibility. Request expansion induces strict binary flips in 9.1%/8.0% of Nimble's judgments and changes 21.4%/18.9% of selection-or-abstention actions in TREC DL2019/2020 under a threshold of 0.5 fixed before inference. Correct-action rates change by 0.0/+8.2 percentage points, respectively, with 95% query-bootstrap intervals of [-6.0,6.0] and [3.8,12.6]. Field masking traces all 70 request-set flips to the schema fields serialized into each scoring prompt. In Von, fixing a shared separator's position eliminates two eligibility-induced preference flips in selected diagnostic states. Laya-typed's default CUDA path produces five passage swaps without strict binary flips, and both yearly action-change intervals include zero; in an FP32 rerun, its probability movement vanishes at the model's four-decimal reporting resolution.

==> native.tex <==
% Generated by build_native.py.
Laya general & 2019 & 0.6 [0.0, 1.4] & 10.8 [6.0, 16.5] & 66.4 [63.5, 68.9] & 0.0$^{\dagger}$ \\
Laya general & 2020 & 0.8 [0.0, 1.9] & 8.0 [4.4, 11.9] & 63.9 [60.4, 67.3] & 2.5 [0.6, 5.0] \\
Laya typed & 2019 & 0.0$^{\dagger}$ & 13.1 [8.3, 18.5] & 66.1 [61.8, 70.1] & 1.7 [0.0, 4.3] \\
Laya typed & 2020 & 0.0$^{\dagger}$ & 15.1 [10.3, 20.1] & 64.8 [61.4, 67.7] & 1.9 [0.0, 4.4] \\
Kev-0.8B & 2019 & 0.0$^{\dagger}$ & 9.4 [5.7, 13.1] & 51.0 [45.6, 56.7] & 0.0$^{\dagger}$ \\
Kev-0.8B & 2020 & 0.0$^{\dagger}$ & 9.6 [6.7, 12.8] & 53.2 [47.8, 58.7] & 0.0$^{\dagger}$ \\
Kev-4B & 2019 & 0.0$^{\dagger}$ & 5.1 [3.1, 7.4] & 75.2 [69.2, 80.9] & 0.0$^{\dagger}$ \\
Kev-4B & 2020 & 0.0$^{\dagger}$ & 5.2 [2.9, 8.0] & 80.1 [74.6, 84.9] & 0.0$^{\dagger}$ \\
Kev-9B & 2019 & 0.0$^{\dagger}$ & 2.8 [1.1, 4.8] & 78.1 [72.6, 82.9] & 0.0$^{\dagger}$ \\
Kev-9B & 2020 & 0.0$^{\dagger}$ & 3.4 [1.7, 5.0] & 85.3 [80.5, 89.7] & 0.0$^{\dagger}$ \\
Nimble-9B & 2019 & 9.1 [6.0, 12.8] & 4.0 [2.3, 6.0] & 74.1 [67.8, 79.8] & 21.4 [15.4, 28.2] \\
Nimble-9B & 2020 & 8.0 [5.2, 11.3] & 2.5 [1.3, 4.0] & 77.1 [73.6, 80.9] & 18.9 [12.6, 25.8] \\
Von 1.2 & 2019 & 0.0$^{\dagger}$ & 2.8 [0.3, 5.7] & 37.0 [34.2, 40.5] & 0.0$^{\dagger}$ \\
Von 1.2 & 2020 & 0.0$^{\dagger}$ & 4.2 [1.5, 7.3] & 40.9 [37.1, 45.1] & 0.0$^{\dagger}$ \\


==> native_class_quality.tex <==
% Generated by build_native.py.
Laya general & 2019 & 40.2 [28.2, 53.0] & 79.5 [72.6, 85.9] & 59.8 \\
Laya general & 2020 & 32.1 [21.4, 42.8] & 79.9 [72.3, 86.5] & 56.0 \\
Laya typed & 2019 & 51.3 [37.6, 65.8] & 73.5 [64.5, 81.6] & 62.4 \\
Laya typed & 2020 & 45.9 [35.8, 56.6] & 74.2 [66.4, 81.4] & 60.1 \\
Kev-0.8B & 2019 & 92.3 [86.3, 96.6] & 30.3 [21.4, 39.7] & 61.3 \\
Kev-0.8B & 2020 & 86.2 [79.2, 92.5] & 36.8 [28.3, 45.3] & 61.5 \\
Kev-4B & 2019 & 67.5 [56.4, 78.6] & 79.1 [70.5, 86.8] & 73.3 \\
Kev-4B & 2020 & 81.1 [72.3, 88.7] & 79.6 [72.3, 85.8] & 80.3 \\
Kev-9B & 2019 & 63.2 [51.3, 75.2] & 85.5 [78.2, 91.5] & 74.4 \\
Kev-9B & 2020 & 78.0 [68.6, 86.8] & 89.0 [84.0, 93.4] & 83.5 \\
Nimble-9B & 2019 & 37.6 [26.5, 48.7] & 92.3 [86.3, 97.0] & 65.0 \\
Nimble-9B & 2020 & 41.5 [32.7, 50.9] & 95.0 [92.1, 97.5] & 68.2 \\
Von 1.2 & 2019 & 98.3 [94.9, 100.0] & 6.4 [2.1, 11.5] & 52.4 \\
Von 1.2 & 2020 & 95.6 [91.2, 98.7] & 13.5 [7.5, 20.4] & 54.6 \\


==> native_contracts.tex <==
% Generated by build_native.py.
Laya general & 2019 & 0.0 & 0.0 & 16.0 & 46.4 & 5.1 & 9.4 \\
Laya general & 2020 & 0.0 & 0.0 & 10.1 & 45.7 & 6.3 & 8.2 \\
Laya typed & 2019 & 0.0 & 0.0 & 15.7 & 59.5 & 3.4 & 4.3 \\
Laya typed & 2020 & 0.0 & 0.0 & 23.7 & 57.0 & 5.0 & 5.7 \\
Kev-0.8B & 2019 & 0.0 & 0.0 & 15.4 & 37.9 & 6.0 & 0.0 \\
Kev-0.8B & 2020 & 0.0 & 0.0 & 21.2 & 35.4 & 6.9 & 0.0 \\
Kev-4B & 2019 & 0.0 & 0.0 & 18.8 & 12.3 & 5.1 & 0.0 \\
Kev-4B & 2020 & 0.0 & 0.0 & 12.8 & 14.0 & 5.0 & 0.0 \\
Kev-9B & 2019 & 0.0 & 0.0 & 17.4 & 8.8 & 4.3 & 0.0 \\
Kev-9B & 2020 & 0.0 & 0.0 & 21.2 & 6.3 & 5.7 & 0.0 \\
Nimble-9B & 2019 & 12.5 & 9.1 & 18.2 & 27.4 & 14.5 & 6.0 \\
Nimble-9B & 2020 & 12.6 & 6.9 & 17.0 & 25.4 & 15.1 & 3.1 \\
Von 1.2 & 2019 & 0.0 & 0.0 & 2.6 & 2.0 & 0.0 & 0.0 \\
Von 1.2 & 2020 & 0.0 & 0.0 & 4.0 & 4.4 & 0.0 & 1.3 \\


==> native_probability.tex <==
% Generated by build_native.py.
Laya general & 2019 & 0.00212 & 0.0709 & 0.0747 \\
Laya general & 2020 & 0.00237 & 0.0678 & 0.0692 \\
Laya typed & 2019 & 0.00134 & 0.0405 & 0.0438 \\
Laya typed & 2020 & 0.00151 & 0.0508 & 0.0384 \\
Kev-0.8B & 2019 & $5.43\times10^{-7}$ & 0.0493 & 0.000471 \\
Kev-0.8B & 2020 & $5.97\times10^{-7}$ & 0.05 & 0.000354 \\
Kev-4B & 2019 & $6.24\times10^{-7}$ & 0.0437 & 0.00226 \\
Kev-4B & 2020 & $6.53\times10^{-7}$ & 0.0445 & 0.00211 \\
Kev-9B & 2019 & $5.77\times10^{-7}$ & 0.0349 & 0.00277 \\
Kev-9B & 2020 & $5.03\times10^{-7}$ & 0.0352 & 0.00222 \\
Nimble-9B & 2019 & 0.102 & 0.0416 & 0.0346 \\
Nimble-9B & 2020 & 0.0951 & 0.037 & 0.0322 \\
Von 1.2 & 2019 & 0 & 0.0155 & 0.0194 \\
Von 1.2 & 2020 & 0 & 0.0193 & 0.0155 \\


==> native_quality.tex <==
% Generated by build_native.py.
Laya general & 2019 & 66.4 & 0.216 & 54.7 & 92.3 & 28.2 & 43.6 \\
Laya general & 2020 & 63.9 & 0.236 & 44.7 & 83.0 & 20.8 & 30.2 \\
Laya typed & 2019 & 66.1 & 0.218 & 59.8 & 82.1 & 41.0 & 56.4 \\
Laya typed & 2020 & 64.8 & 0.222 & 52.2 & 83.0 & 26.4 & 47.2 \\
Kev-0.8B & 2019 & 51.0 & 0.285 & 52.1 & 7.7 & 61.5 & 87.2 \\
Kev-0.8B & 2020 & 53.2 & 0.278 & 53.5 & 17.0 & 58.5 & 84.9 \\
Kev-4B & 2019 & 75.2 & 0.173 & 63.2 & 53.8 & 53.8 & 82.1 \\
Kev-4B & 2020 & 80.1 & 0.148 & 74.8 & 60.4 & 73.6 & 90.6 \\
Kev-9B & 2019 & 78.1 & 0.157 & 65.0 & 56.4 & 59.0 & 79.5 \\
Kev-9B & 2020 & 85.3 & 0.111 & 76.1 & 60.4 & 79.2 & 88.7 \\
Nimble-9B & 2019 & 74.1 & 0.210 & 58.1 & 84.6 & 38.5 & 51.3 \\
Nimble-9B & 2020 & 77.1 & 0.178 & 62.3 & 84.9 & 47.2 & 54.7 \\
Von 1.2 & 2019 & 37.0 & 0.315 & 40.2 & 10.3 & 48.7 & 61.5 \\
Von 1.2 & 2020 & 40.9 & 0.305 & 40.3 & 20.8 & 32.1 & 67.9 \\


==> native_quality_controls.tex <==
% Generated by build_native.py.
Qwen3.5-4B control & 2019 & 67.5 & 0.242 & 64.1 & 30.8 & 74.4 & 87.2 \\
Qwen3.5-4B control & 2020 & 73.4 & 0.190 & 71.1 & 34.0 & 84.9 & 94.3 \\
Qwen3.5-9B control & 2019 & 76.4 & 0.186 & 70.9 & 48.7 & 76.9 & 87.2 \\
Qwen3.5-9B control & 2020 & 83.6 & 0.126 & 75.5 & 56.6 & 77.4 & 92.5 \\
Llama3.1-8B control & 2019 & 34.2 & 0.480 & 55.6 & 0.0 & 69.2 & 97.4 \\
Llama3.1-8B control & 2020 & 34.8 & 0.483 & 56.0 & 0.0 & 77.4 & 90.6 \\
Qwen2.5-1.5B control & 2019 & 70.4 & 0.199 & 50.4 & 79.5 & 20.5 & 51.3 \\
Qwen2.5-1.5B control & 2020 & 68.8 & 0.210 & 43.4 & 79.2 & 17.0 & 34.0 \\


==> native_thresholds_2019.tex <==
% Generated by build_native.py.
Laya general & 0.5 & 54.7 & 54.7 & 31.6 & 31.6 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.7 & 47.0 & 47.0 & 15.4 & 15.4 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.9 & 33.3 & 33.3 & 0.0$^{\ddagger}$ & 0.0$^{\ddagger}$ & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
Laya typed & 0.5 & 59.8 & 59.0 & 43.6 & 43.6 & 1.7 [0.0, 4.3] & -0.9 [-2.6, 0.0] \\
 & 0.7 & 33.3 & 33.3 & 0.0$^{\ddagger}$ & 0.0$^{\ddagger}$ & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.9 & 33.3 & 33.3 & 0.0$^{\ddagger}$ & 0.0$^{\ddagger}$ & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
Kev-0.8B & 0.5 & 52.1 & 52.1 & 94.9 & 94.9 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.7 & 57.3 & 57.3 & 73.5 & 73.5 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.9 & 39.3 & 39.3 & 9.4 & 9.4 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
Kev-4B & 0.5 & 63.2 & 63.2 & 70.1 & 70.1 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.7 & 63.2 & 63.2 & 52.1 & 52.1 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.9 & 51.3 & 51.3 & 21.4 & 21.4 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
Kev-9B & 0.5 & 65.0 & 65.0 & 63.2 & 63.2 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.7 & 65.0 & 65.0 & 56.4 & 56.4 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.9 & 66.7 & 66.7 & 48.7 & 48.7 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
Nimble-9B & 0.5 & 58.1 & 58.1 & 41.9 & 54.7 & 21.4 [15.4, 28.2] & 0.0 [-6.0, 6.0] \\
 & 0.7 & 54.7 & 58.1 & 32.5 & 44.4 & 19.7 [12.0, 28.2] & +3.4 [-2.6, 9.4] \\
 & 0.9 & 48.7 & 52.1 & 23.9 & 33.3 & 16.2 [9.4, 23.9] & +3.4 [-1.7, 8.5] \\
Von 1.2 & 0.5 & 40.2 & 40.2 & 95.7 & 95.7 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.7 & 32.5 & 32.5 & 3.4 & 3.4 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.9 & 33.3 & 33.3 & 0.0$^{\ddagger}$ & 0.0$^{\ddagger}$ & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\


==> native_thresholds_2020.tex <==
% Generated by build_native.py.
Laya general & 0.5 & 44.7 & 44.7 & 27.0 & 26.4 & 2.5 [0.6, 5.0] & 0.0 [-1.9, 1.9] \\
 & 0.7 & 42.1 & 42.8 & 12.6 & 13.2 & 0.6 [0.0, 1.9] & +0.6 [0.0, 1.9] \\
 & 0.9 & 33.3 & 33.3 & 0.0$^{\ddagger}$ & 0.0$^{\ddagger}$ & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
Laya typed & 0.5 & 52.2 & 52.8 & 39.0 & 39.0 & 1.9 [0.0, 4.4] & +0.6 [0.0, 1.9] \\
 & 0.7 & 33.3 & 33.3 & 0.0$^{\ddagger}$ & 0.0$^{\ddagger}$ & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.9 & 33.3 & 33.3 & 0.0$^{\ddagger}$ & 0.0$^{\ddagger}$ & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
Kev-0.8B & 0.5 & 53.5 & 53.5 & 91.2 & 91.2 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.7 & 55.3 & 55.3 & 65.4 & 65.4 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.9 & 39.6 & 39.6 & 8.2 & 8.2 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
Kev-4B & 0.5 & 74.8 & 74.8 & 74.2 & 74.2 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.7 & 72.3 & 72.3 & 56.6 & 56.6 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.9 & 56.0 & 56.0 & 27.0 & 27.0 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
Kev-9B & 0.5 & 76.1 & 76.1 & 72.3 & 72.3 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.7 & 75.5 & 75.5 & 66.0 & 66.0 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.9 & 79.2 & 79.2 & 56.0 & 56.0 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
Nimble-9B & 0.5 & 62.3 & 70.4 & 42.8 & 50.9 & 18.9 [12.6, 25.8] & +8.2 [3.8, 12.6] \\
 & 0.7 & 60.4 & 67.9 & 35.8 & 44.7 & 18.2 [12.6, 24.5] & +7.5 [3.1, 12.6] \\
 & 0.9 & 58.5 & 61.6 & 29.6 & 34.0 & 16.4 [10.1, 23.3] & +3.1 [-2.5, 8.8] \\
Von 1.2 & 0.5 & 40.3 & 40.3 & 90.6 & 90.6 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.7 & 34.6 & 34.6 & 6.3 & 6.3 & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\
 & 0.9 & 33.3 & 33.3 & 0.0$^{\ddagger}$ & 0.0$^{\ddagger}$ & 0.0$^{\dagger}$ & 0.0$^{\dagger}$ \\


==> original.tex <==
% Generated by build_results.py; do not hand-edit.
Qwen3.5-4B & 2019 & 23.1 [17.7, 28.8] & 22.5 [17.4, 27.9] & 5.4 [2.8, 8.3] \\
Qwen3.5-4B & 2020 & 22.6 [18.2, 27.0] & 18.0 [14.5, 21.8] & 3.4 [1.9, 5.0] \\
Qwen3.5-9B & 2019 & 14.0 [10.5, 17.7] & 13.7 [10.3, 17.4] & 2.6 [1.1, 4.0] \\
Qwen3.5-9B & 2020 & 13.6 [10.3, 17.2] & 16.1 [13.2, 19.5] & 3.8 [2.3, 5.5] \\
Llama3.1-8B & 2019 & 23.1 [18.8, 27.4] & 49.6 [45.3, 53.8] & 6.6 [4.0, 9.1] \\
Llama3.1-8B & 2020 & 23.1 [18.2, 28.3] & 50.7 [46.1, 55.3] & 9.6 [6.3, 13.6] \\
Qwen2.5-1.5B* & 2019 & 17.1 [13.1, 21.1] & 32.8 [29.1, 36.2] & 13.4 [9.4, 17.7] \\
Qwen2.5-1.5B* & 2020 & 20.8 [17.2, 24.3] & 32.5 [27.9, 36.9] & 13.0 [9.6, 16.8] \\


==> results.tex <==
% Generated by build_results.py; do not hand-edit.
Qwen3.5-4B & 2019 & 17.1 [12.8, 21.4] & 24.8 [19.7, 29.9] & 4.3 [2.0, 6.8] & 6.6 [2.6, 10.3] \\
Qwen3.5-4B & 2020 & 12.8 [10.1, 15.7] & 19.5 [15.5, 23.7] & 6.5 [4.2, 9.0] & 5.0 [1.7, 8.2] \\
Qwen3.5-9B & 2019 & 16.0 [11.7, 20.5] & 19.7 [15.4, 23.9] & 3.4 [1.7, 5.7] & 2.8 [-1.1, 6.8] \\
Qwen3.5-9B & 2020 & 15.9 [12.6, 19.5] & 17.0 [14.3, 19.9] & 5.9 [3.8, 8.2] & -3.8 [-7.5, 0.2] \\
Llama3.1-8B & 2019 & 9.4 [6.0, 13.4] & 53.3 [49.6, 57.0] & 0.9 [0.0, 2.3] & 10.5 [6.8, 14.8] \\
Llama3.1-8B & 2020 & 11.5 [8.6, 14.7] & 53.7 [50.5, 56.6] & 1.3 [0.4, 2.5] & 11.7 [8.4, 15.3] \\
Qwen2.5-1.5B* & 2019 & 18.8 [14.8, 22.8] & 21.7 [17.7, 25.6] & 7.4 [4.6, 10.3] & -4.3 [-9.4, 1.1] \\
Qwen2.5-1.5B* & 2020 & 17.2 [13.2, 21.6] & 22.9 [19.9, 25.8] & 7.3 [4.8, 10.3] & -7.3 [-11.5, -3.4] \\


==> scenarios.tex <==
% Generated by build_results.py; do not hand-edit.
Qwen3.5-4B & 2019 & Zero & 30.77 & 38.46 & 28.21 & 48.72 & 51.28 \\
Qwen3.5-4B & 2019 & One & 74.36 & 74.36 & 69.23 & 66.67 & 71.79 \\
Qwen3.5-4B & 2019 & Two & 87.18 & 87.18 & 92.31 & 89.74 & 87.18 \\
Qwen3.5-4B & 2020 & Zero & 33.96 & 32.08 & 28.30 & 56.60 & 67.92 \\
Qwen3.5-4B & 2020 & One & 84.91 & 69.81 & 69.81 & 81.13 & 67.92 \\
Qwen3.5-4B & 2020 & Two & 94.34 & 98.11 & 92.45 & 92.45 & 92.45 \\
Qwen3.5-9B & 2019 & Zero & 48.72 & 35.90 & 12.82 & 38.46 & 48.72 \\
Qwen3.5-9B & 2019 & One & 76.92 & 74.36 & 71.79 & 74.36 & 82.05 \\
Qwen3.5-9B & 2019 & Two & 87.18 & 89.74 & 92.31 & 84.62 & 89.74 \\
Qwen3.5-9B & 2020 & Zero & 56.60 & 37.74 & 26.42 & 54.72 & 67.92 \\
Qwen3.5-9B & 2020 & One & 77.36 & 81.13 & 81.13 & 75.47 & 75.47 \\
Qwen3.5-9B & 2020 & Two & 92.45 & 90.57 & 94.34 & 92.45 & 92.45 \\
Llama3.1-8B & 2019 & Zero & 0.00 & 2.56 & 0.00 & 0.00 & 20.51 \\
Llama3.1-8B & 2019 & One & 69.23 & 58.97 & 46.15 & 58.97 & 48.72 \\
Llama3.1-8B & 2019 & Two & 97.44 & 79.49 & 69.23 & 92.31 & 84.62 \\
Llama3.1-8B & 2020 & Zero & 0.00 & 0.00 & 0.00 & 0.00 & 15.09 \\
Llama3.1-8B & 2020 & One & 77.36 & 50.94 & 35.85 & 73.58 & 37.74 \\
Llama3.1-8B & 2020 & Two & 90.57 & 81.13 & 71.70 & 94.34 & 77.36 \\
Qwen2.5-1.5B* & 2019 & Zero & 79.49 & 0.00 & 0.00 & 0.00 & 0.00 \\
Qwen2.5-1.5B* & 2019 & One & 20.51 & 53.85 & 46.15 & 66.67 & 64.10 \\
Qwen2.5-1.5B* & 2019 & Two & 51.28 & 69.23 & 66.67 & 87.18 & 87.18 \\
Qwen2.5-1.5B* & 2020 & Zero & 79.25 & 0.00 & 0.00 & 5.66 & 5.66 \\
Qwen2.5-1.5B* & 2020 & One & 16.98 & 45.28 & 43.40 & 58.49 & 56.60 \\
Qwen2.5-1.5B* & 2020 & Two & 33.96 & 81.13 & 71.70 & 90.57 & 88.68 \\


==> sensitivity.tex <==
% Generated by build_results.py; do not hand-edit.
Qwen3.5-4B & 2019 & 23.1 [18.5, 27.9] & 10.5 [6.8, 14.5] & 14.0 [10.5, 17.7] & 18.8 [13.4, 24.2] \\
Qwen3.5-4B & 2020 & 21.8 [18.2, 25.6] & 11.7 [8.8, 14.9] & 15.3 [11.9, 19.1] & 20.3 [15.5, 25.6] \\
Qwen3.5-9B & 2019 & 16.8 [12.5, 21.4] & 9.4 [5.7, 13.7] & 19.9 [15.4, 24.5] & 11.7 [8.0, 15.7] \\
Qwen3.5-9B & 2020 & 15.5 [12.2, 19.1] & 8.0 [5.7, 10.3] & 19.7 [15.5, 24.1] & 13.0 [9.9, 16.4] \\
Llama3.1-8B & 2019 & 9.7 [6.3, 13.4] & 5.4 [3.1, 8.0] & 23.6 [17.4, 30.2] & 0.3 [0.0, 0.9] \\
Llama3.1-8B & 2020 & 12.2 [8.8, 15.7] & 7.8 [5.5, 10.1] & 21.6 [17.4, 25.8] & 1.5 [0.2, 2.9] \\
Qwen2.5-1.5B* & 2019 & 53.0 [46.7, 59.0] & 19.1 [16.0, 22.5] & 15.1 [10.8, 19.7] & 48.7 [42.5, 55.0] \\
Qwen2.5-1.5B* & 2020 & 62.9 [56.6, 68.8] & 17.2 [13.8, 20.5] & 9.6 [6.3, 13.2] & 56.6 [51.2, 62.1] \\


==> support.tex <==
% Generated by build_results.py; do not hand-edit.
Qwen3.5-4B & 2019 & 96.99 & 99.87 & 23.1 [17.7, 28.8] & 17.1 [12.8, 21.4] \\
Qwen3.5-4B & 2020 & 96.84 & 99.86 & 22.6 [18.2, 27.0] & 12.8 [10.1, 15.7] \\
Qwen3.5-9B & 2019 & 97.85 & 99.85 & 14.0 [10.5, 17.7] & 16.0 [11.7, 20.5] \\
Qwen3.5-9B & 2020 & 97.61 & 99.85 & 13.6 [10.3, 17.2] & 15.9 [12.6, 19.5] \\
Llama3.1-8B & 2019 & 0.55 & 99.82 & 23.1 [18.8, 27.4] & 9.4 [6.0, 13.4] \\
Llama3.1-8B & 2020 & 0.61 & 99.85 & 23.1 [18.2, 28.3] & 11.5 [8.6, 14.7] \\
Qwen2.5-1.5B* & 2019 & 99.58 & 99.99 & 17.1 [13.1, 21.1] & 18.8 [14.8, 22.8] \\
Qwen2.5-1.5B* & 2020 & 99.18 & 99.93 & 20.8 [17.2, 24.3] & 17.2 [13.2, 21.6] \\


==> workflow.tex <==
% Generated by build_results.py; do not hand-edit.
Qwen3.5-4B & 2019 & 28.2 [20.5, 35.9] & 34.2 [25.6, 43.6] & 30.77 & 38.46 & 51.28 \\
Qwen3.5-4B & 2020 & 30.8 [23.3, 38.4] & 29.6 [23.3, 36.5] & 33.96 & 32.08 & 67.92 \\
Qwen3.5-9B & 2019 & 23.9 [17.1, 30.8] & 30.8 [23.1, 39.3] & 48.72 & 35.90 & 48.72 \\
Qwen3.5-9B & 2020 & 21.4 [15.7, 27.7] & 28.3 [20.8, 36.5] & 56.60 & 37.74 & 67.92 \\
Llama3.1-8B & 2019 & 38.5 [29.9, 47.0] & 36.8 [28.2, 45.3] & 0.00 & 2.56 & 20.51 \\
Llama3.1-8B & 2020 & 34.0 [26.4, 42.1] & 40.9 [33.3, 49.1] & 0.00 & 0.00 & 15.09 \\
Qwen2.5-1.5B* & 2019 & 35.9 [25.6, 47.0] & 24.8 [16.2, 33.3] & 79.49 & 0.00 & 0.00 \\
Qwen2.5-1.5B* & 2020 & 49.1 [39.6, 58.5] & 34.6 [26.4, 42.8] & 79.25 & 0.00 & 5.66 \\

